Model-Augmented Actor-Critic: Backpropagating through Paths

Current model-based reinforcement learning approaches use the model simply as a learned black-box simulator to augment the data for policy optimization or value function learning. In this paper, we show how to make more effective use of the model by exploiting its differentiability. We construct a policy optimization algorithm that uses the pathwise derivative of the learned model and policy across future timesteps. Instabilities of learning across many timesteps are prevented by using a terminal value function, learning the policy in an actor-critic fashion. Furthermore, we present a derivation on the monotonic improvement of our objective in terms of the gradient error in the model and value function. We show that our approach (i) is consistently more sample efficient than existing state-of-the-art model-based algorithms, (ii) matches the asymptotic performance of model-free algorithms, and (iii) scales to long horizons, a regime where typically past model-based approaches have struggled.

==> Model-Based Done Right/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Model-Based Done Right/sections/01_introduction.tex <==

\section{Introduction}

Model-based reinforcement learning (RL) offers the potential to be a general-purpose tool for learning complex policies while being sample efficient. When learning in real-world physical systems, data collection can be an arduous process. Contrary to model-free methods, model-based approaches are appealing due to their comparatively fast learning. By first learning the dynamics of the system in a supervised learning way, it can exploit off-policy data. Then, model-based methods use the model to derive controllers from it either parametric controllers~\citep{luo2018algorithmic, buckman2018steve, janner2019mbpo} or non-parametric controllers~\citep{nagabandi2017neural, chua2018deep}.

Current model-based methods learn with an order of magnitude less data than their model-free counterparts while achieving the same asymptotic convergence. Tools like ensembles, probabilistic models, planning over shorter horizons, and meta-learning have been used to achieved such performance~\citep{kurutach2018model, chua2018deep, clavera2018mbmpo}. However, the model usage in all of these methods is the same: simple data augmentation. They use the learned model as a black-box simulator generating samples from it. In high-dimensional environments or environments that require longer planning, substantial sampling is needed to provide meaningful signal for the policy. \textit{Can we further exploit our learned models?}

In this work, we propose to estimate the policy gradient by backpropagating its gradient through the model using the pathwise derivative estimator. Since the learned model is differentiable, one can link together the model, reward function, and policy to obtain an analytic expression for the gradient of the returns with respect to the policy. By computing the gradient in this manner, we obtain an expressive signal that allows rapid policy learning. We avoid the instabilities that often result from back-propagating through long horizons by using a terminal Q-function. This scheme fully exploits the learned model without harming the learning stability seen in previous approaches~\citep{kurutach2018model,heess2015learning}. The horizon at which we apply the terminal Q-function acts as a hyperparameter between model-free (when fully relying on the Q-function) and model-based (when using a longer horizon) of our algorithm.

The main contribution of this work is a model-based method that significantly reduces the sample complexity compared to state-of-the-art model-based algorithms~\citep{janner2019mbpo, buckman2018steve}. For instance, we achieve a 10k return in the half-cheetah environment in just 50 trajectories. We theoretically justify our optimization objective and derive the monotonic improvement of our learned policy in terms of the Q-function and the model error. Furtermore, we experimentally analyze the theoretical derivations. Finally, we pinpoint the importance of our objective by ablating all the components of our algorithm. The results are reported in four model-based benchmarking environments~\citep{wang2019mbbench, 2012mujoco}. The low sample complexity and high performance of our method carry high promise towards learning directly on real robots.

==> Model-Based Done Right/sections/02_related_work.tex <==
\vspace{-0.1in}
\section{Related Work}
\vspace{-0.1in}

\textbf{Model-Based Reinforcement Learning. } Learned dynamics models offer the possibility to reduce sample complexity while maintaining the asymptotic performance. For instance, the models can act as a learned simulator on which a model-free policy is trained on~\citep{kurutach2018model, luo2018algorithmic, janner2019mbpo}. The model can also be used to improve the target value estimates~\citep{feinberg2018model} or to provide additional context to a policy~\citep{Du2019prior}. Contrary to these methods, our approach uses the model in a different way: we exploit the fact that the learned simulator is differentiable and optimize the policy with the analytical gradient.
Long term predictions suffer from a compounding error effect in the model, resulting in unrealistic predictions. In such cases, the policy tends to overfit to the deficiencies of the model, which translates to poor performance in the real environment; this problem is known as model-bias~\citep{deisenroth2011pilco}. The model-bias problem has motivated work that uses meta-learning~\citep{clavera2018mbmpo}, interpolation between different horizon predictions~\citep{buckman2018steve, janner2019mbpo}, and interpolating between model and real data~\citep{kalweit2017uncertainty}. To prevent model-bias, we exploit the model for a short horizon and use a terminal value function to model the rest of the trajectory. Finally, since our approach returns a stochastic policy, dynamics model, and value function could use model-predictive control (MPC) for better performance at test time, similar to ~\citep{lowrey2018polo, Hong2019ModelbasedLR}. MPC methods~\citep{nagabandi2017neural} have shown to be very effective when the uncertainty of the dynamics is modelled~\citep{chua2018deep, wang2019lookahead}.

\textbf{Differentable Planning. } Previous work has used backpropagate through learned models to obtain the optimal sequences of actions. For instance,~\cite{levine2014learning} learn linear local models and obtain the optimal sequences of actions, which is then distilled into a neural network policy. The planning can be incorporated into the neural network architecture~\citep{okada2017path, tamar2016vin, srinivas2018universal, karkus209diffalg} or formulated as a differentiable function~\citep{pereira2018mpcnn, br2018differentiable}. Planning sequences of actions, even when doing model-predictive control (MPC), does not scale well to high-dimensional, complex domains~\cite{janner2019mbpo}. Our method, instead learns a neural network policy in an actor-critic fashion aided with a learned model. In our study, we evaluate the benefit of carrying out MPC on top of our learned policy at test time, Section~\ref{sec:mpc}. The results suggest that the policy captures the optimal sequence of action, and re-planning does not result in significant benefits.


\textbf{Policy Gradient Estimation. } The reinforcement learning objective involves computing the gradient of an expectation~\citep{schulman2015graphs}. By using Gaussian processes~\citep{deisenroth2011pilco}, it is possible to compute the expectation analytically. However, when learning expressive parametric non-linear dynamical models and policies, such closed form solutions do not exist. The gradient is then estimated using Monte-Carlo methods~\citep{mohamed2019monte}. In the context of model-based RL, previous approaches mostly made use of the score-function, or REINFORCE estimator~\citep{peters2006pg, kurutach2018model}. However, this estimator has high variance and extensive sampling is needed, which hampers its applicability in high-dimensional environments. In this work, we make use of the pathwise derivative estimator~\citep{mohamed2019monte}. Similar to our approach,~\citet{heess2015learning} uses this estimator in the context of model-based RL. However, they just make use of real-world trajectories that introduces the need of a likelihood ratio term for the model predictions, which in turn increases the variance of the gradient estimate. Instead, we entirely rely on the predictions of the model, removing the need of likelihood ratio terms.

\textbf{Actor-Critic Methods. } Actor-critic methods alternate between policy evaluation, computing the value function for the policy; and policy improvement using such value function~\citep{sutton1998rl, barto1983neuro}. Actor-critic methods can be classified between on-policy and off-policy. On-policy methods tend to be more stable, but at the cost of sample efficiency~\citep{sutton1991planning, mnih2016asynchronous}. On the other hand, off-policy methods offer better sample complexity~\citep{lillicrap2015continuous}. Recent work has significantly stabilized and improved the performance of off-policy methods using maximum-entropy objectives~\citep{haarnoja2018soft} and multiple value functions~\citep{fujimoto2018addressing}.
Our method combines the benefit of both. By using the learned model we can have a learning that resembles an on-policy method while still being off-policy.

% Many actor-critic algorithms build on the standard, on-policy policy gradient formulation to update the actor (Peters & Schaal, 2008), and many of them also consider the entropy of the policy, but instead of maximizing the entropy.
% On-policy training tends to improve stability but results in poor sample complexity. There have been efforts to increase the sample efficiency while retaining robustness by incorporating off-policy samples and by using higher order variance reduction techniques (O’Donoghue et al., 2016; Gu et al., 2016).
% However, fully off-policy algorithms still attain better efficiency. A particularly popular off-policy actor-critic method, DDPG (Lillicrap et al., 2015), which is a deep variant of the deterministic policy gradient (Silver et al., 2014) algorithm, uses a Q-function estimator to enable off-policy learning, and a deterministic actor that maximizes this Q-function. As such, this method can be viewed both as a deterministic actor-critic algorithm and an approximate Q-learning algorithm. 
% Unfortunately, the interplay between the deterministic actor network and the Q-function typically makes DDPG extremely difficult to stabilize and brittle to hyperparameter settings (Duan et al., 2016; Henderson et al., 2017). As a consequence, it is difficult to extend DDPG to complex, high-dimensional tasks, and on-policy policy gradient methods still tend to produce the best results in such settings (Gu et al., 2016). Our method instead combines off-policy actor-critic training with a stochastic actor, and further aims to maximize the entropy of this actor with an entropy maximization objective. We find that this actually results in a considerably more stable and scalable algorithm that, in practice, exceeds both the efficiency and final performance of DDPG. A similar method can be derived as a zero-step special case of stochastic value gradients (SVG(0)) (Heess et al., 2015). However, SVG(0) differs from our method in that it optimizes the standard maximum expected return
% objective.


==> Model-Based Done Right/sections/03_background.tex <==

\section{Background}

In this section, we present the reinforcement learning problem, two different lines of algorithms that tackle it, and a summary on Monte-Carlo gradient estimators.
\subsection{Reinforcement Learning} \label{sec:back-rl}
A discrete-time finite Markov decision process (MDP) $\mathcal{M}$ is  defined by the tuple $(\mathcal{S}, \mathcal{A}, f, r, \gamma, p_0, T)$. 
Here, $\mathcal{S}$ is the set of states, $\mathcal{A}$ the action space, $s_{t+1}\sim f(s_t, a_t)$ the transition distribution,
$r: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}$ is a reward function, $p_0: \mathcal{S} \to \mathbb{R}_+$ represents the initial state distribution, $\gamma$ the discount factor, and $T$ is the horizon of the process. We define the return as the sum of rewards $r(s_t, a_t)$ along a trajectory $\tau := (s_{0}, a_{0}, ..., s_{T-1}, a_{T-1}, s_{T})$. The goal of reinforcement learning is to find a policy $\pi_{\bm{\theta}}: \mathcal{S} \times \mathcal{A} \rightarrow \mathbb{R}^+$ that maximizes the expected return, i.e., $\max_{\bm{\theta}} J(\bm{\theta}) = \max_{\bm{\theta}} \mathbb{E}[\sum_t \gamma^t r(s_t, a_t)]$.

\textbf{Actor-Critic.} In actor-critic methods, we learn a function $\hat{Q}$ (critic) that approximates the expected return conditioned on a state $s$ and action $a$, $ \mathbb{E}[\sum_t \gamma^t r(s_t, a_t)|s_0=s, a_0=a]$. Then, the learned Q-function is used to optimize a policy $\pi$ (actor). Usually, the Q-function is learned by iteratively minimizing the Bellman residual:
\begin{align*}
    J_{Q} = \mathbb{E}[(\hat{Q}(s_t, a_t) - (r(s_t, a_t) + \gamma \hat{Q}(s_{t+1}, a_{t+1})))^2]
\end{align*}
% 
The above method is referred as one-step Q-learning, and while a naive implementation often results in unstable behaviour, recent methods have succeeded in stabilizing the Q-function training~\citep{fujimoto2018addressing}. The actor then can be trained to maximize the learned $\hat{Q}$ function $
J_\pi = \mathbb{E} \left[ \hat{Q}(s,\pi(s)) \right]
$. The benefit of this form of actor-critic method is that it can be applied in an off-policy fashion, sampling random mini-batches of transitions from an experience replay buffer~\citep{Lin1992}.

\textbf{Model-Based RL. } Model-based methods, contrary to model-free RL, learn the transition distribution from experience. Typically, this is carried out by learning a parametric function approximator $\hat{f}_{\bm{\phi}}$, known as a dynamics model. We define the state predicted by the dynamics model as $\hat{s}_{t+1}$, i.e., $\hat{s}_{t+1} \sim \hat{f}_{\bm{\phi}}(s_{t}, a_t)$. The models are trained via maximum likelihood: $\max_{\bm{\phi}} J_{f}(\bm{\phi}) = \max_{\bm{\phi}} \mathbb{E}[\log p(\hat{s}_{t+1}|s_t, a_t) ]$

\subsection{Monte-Carlo Gradient Estimators}
In order to optimize the reinforcement learning objective, it is needed to take the gradient of an expectation. In general, it is not possible to compute the exact expectation so Monte-Carlo gradient estimators are used instead. These are mainly categorized into three classes: the pathwise, score function, and measure-valued gradient estimator~\citep{mohamed2019monte}. In this work, we use the pathwise gradient estimator, which is also known as the re-parameterization trick~\citep{kingma2013auto}. This estimator is derived from the law of the unconscious statistician (LOTUS)~\citep{grimmett2001probability}
% 
\begin{align*}
    \mathbb{E}_{p_{\bm{\theta}}(x)}[f(x)] = \mathbb{E}_{p(\epsilon)}[f(g_{\bm{\theta}}(\epsilon)]
\end{align*}
% 
Here, we have stated that we can compute the expectation of a random variable $x$ without knowing its distribution, if we know its corresponding sampling path and base distribution. A common case, and the one used in this manuscript, $\theta$ parameterizes a Gaussian distribution: $x \sim p_{\bm{\theta}} = \mathcal{N}(\mu_\theta, \sigma_\theta^2)$, which is equivalent to  $x = \mu_{\bm{\theta}} + \epsilon \sigma_{\bm{\theta}}$ for $\epsilon \sim \mathcal{N}(0, 1)$.


==> Model-Based Done Right/sections/04_method.tex <==

\section{Policy Gradient via Model-Augmented Pathwise Derivative}


Exploiting the full capability of learned models has the potential to enable complex and high-dimensional real robotics tasks while maintaining low sample complexity. Our approach, model-augmented actor-critic (MAAC), exploits the learned model by computing the analytic gradient of the returns with respect to the policy. 
In contrast to sample-based methods, which one can think of as providing directional derivatives in trajectory space, MAAC computes the full gradient, providing a strong learning signal for policy learning, which further decreases the sample complexity.
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    % \vspace{-0.1in}
    \includegraphics[
    trim={2.5cm 2.cm 1.5cm 0.cm}, clip,
    width=\linewidth]{sections/comp_graph.pdf}
    \caption{\small Stochastic computation graph of the proposed objective $J_\pi$. The stochastic nodes are represented by circles and the deterministic ones by squares.}
    \label{fig:comp_graph}
    \vspace{-0.3in}
\end{wrapfigure}
In the following, we present our policy optimization scheme and describe the full algorithm.


\subsection{Model-Augmented Actor-Critic Objective}
Among model-free methods, actor-critic methods have shown superior performance in terms of sample efficiency and asymptotic performance~\citep{haarnoja2018soft}. However, their sample efficiency remains worse than model-based approaches, and fully off-policy methods still show instabilities comparing to on-policy algorithms~\citep{mnih2016asynchronous}. Here, we propose a modification of the Q-function parametrization by using the model predictions on the first time-steps after the action is taken. Specifically, we do policy optimization by maximizing the following objective:
% 
\begin{align*}
    J_{\pi}(\bm{\theta}) = \mathbb{E}\left[ \sum_{t=0}^{H-1} \gamma^t r(s_t) + \gamma^H \hat{Q}(s_H, a_H)\right]
\end{align*}
% 
whereby, $s_{t+1} \sim \hat{f}(s_t, a_t)$ and $a_t \sim \pi_{\bm{\theta}}(s_t)$. Note that under the true dynamics and Q-function, this objective is the same as the RL objective. Contrary to previous reinforcement learning methods, we optimize this objective by back-propagation through time. Since the learned dynamics model and policy are parameterized as Gaussian distributions, we can make use of the pathwise derivative estimator to compute the gradient, resulting in an objective that captures uncertainty while presenting low variance. The computational graph of the proposed objective is shown in Figure~\ref{fig:comp_graph}.

While the proposed objective resembles n-step bootstrap~\citep{sutton1998rl}, our model usage fundamentally differs from previous approaches. First, we do not compromise between being off-policy and stability. Typically, n-step bootstrap is either on-policy, which harms the sample complexity, or its gradient estimation uses likelihood ratios, which presents large variance and results in unstable learning~\citep{heess2015learning}. Second, we obtain a strong learning signal by  backpropagating the gradient of the policy across multiple steps using the pathwise derivative estimator, instead of the REINFORCE estimator~\citep{mohamed2019monte, peters2006pg}. And finally, we prevent the exploding and vanishing gradients effect inherent to back-propagation through time by the means of the terminal Q-function~\citep{kurutach2018model}.
% \yz{inherited from}

The horizon $H$ in our proposed objective allows us to trade off between the accuracy of our learned model and the accuracy of our learned Q-function. Hence, it controls the degree to which our algorithm is model-based or well model-free.  If we were not to trust our model at all ($H=0$), we would end up with a model-free update; for $H=\infty$, the objective results in a shooting objective. Note that we will perform policy optimization by taking derivatives of the objective, hence we require accuracy on the derivatives of the objective and not on its value. The following lemma provides a bound on the gradient error in terms of the error on the derivatives of the model, the Q-function, and the horizon $H$.

\begin{lemma}[Gradient Error] 
\label{lemma:gradient error}
Let $\hat{f}$ and $\hat{Q}$ be the learned approximation of the dynamics $f$ and Q-function $Q$, respectively. Assume that $Q$ and $\hat{Q}$ have $L_q/2$-Lipschitz continuous gradient and $f$ and $\hat{f}$ have $L_f/2$-Lipschitz continuous gradient. Let $\epsilon_f = \max_{t} \| \nabla \hat{f}(\hat{s}_t, \hat{a}_t) - \nabla f(s_t, a_t)\|_2$ be the error on the model derivatives and $\epsilon_Q = \| \nabla \hat{Q}(\hat{s}_H, \hat{a}_H) - \nabla Q(s_H, a_H)\|_2$ the error on the Q-function derivative. Then the error on the gradient between the learned objective and the true objective can be bounded by:
\begin{align*}
    \mathbb{E}\left[\| \nabla_{\bm{\theta}}J_{\pi} - \nabla_{\bm{\theta}}\hat{J}_{\pi} \|_2\right] \leq c_1(H) \epsilon_f + c_2(H) \epsilon_Q
\end{align*}
\begin{proof}
\vspace{-0.1in}
See Appendix.
\end{proof}
\end{lemma}

The result in Lemma~\ref{lemma:gradient error} stipulates the error of the policy gradient in terms of the maximum error in the model derivatives and the error in the Q derivatives. The functions $c_1$ and $c_2$ are functions of the horizon and depend on the Lipschitz constants of the model and the Q-function. Note that we are just interested in the relation between both sources of error, since the gradient magnitude will be scaled by the learning rate, or by the optimizer, when applying it to the weights.

\subsection{Monotonic Improvement}
In the previous section, we presented our objective and the error it incurs in the policy gradient with respect to approximation error in the model and the Q function. However, the error on the gradient is not indicative of the effect of the desired metric: the average return. Here, we quantify the effect of the modeling error on the return. First, we will bound the KL-divergence between the policies resulting from taking the gradient with the true objective and the approximated one. Then we will bound the performance in terms of the KL.

\begin{lemma}[Total Variation Bound]
\label{lemma: kl bound}
Under the assumptions of the Lemma~\ref{lemma:gradient error}, let $\bm{\theta} = \bm{\theta}_o + \alpha \nabla_{\bm{\theta}}J_{\pi}$ be the parameters resulting from taking a gradient step on the exact objective, and $\bm{\hat{\theta}} = \bm{\theta}_o + \alpha \nabla_{\bm{\theta}}\hat{J}_{\pi}$ the parameters resulting from taking a gradient step on approximated objective, where $\alpha \in \mathbb{R}^+$. Then the following bound on the total variation distance holds
\begin{align*}
    \max_s D_{\text{TV}}(\pi_{\theta}||\pi_{\hat{\theta}}) \leq \alpha c_3 (\epsilon_f c_1(H) + \epsilon_Q c_2(H))
\end{align*}
\begin{proof}
\vspace{-0.1in}
See Appendix.
\end{proof}

\end{lemma}

The previous lemma results in a bound on the distance between the policies originated from taking a gradient step using the true dynamics and Q-function, and using its learned counterparts. Now, we can derive a similar result from ~\citet{Kakade02approximatelyoptimal} to bound the difference in average returns.

\begin{theorem}[Monotonic Improvement] Under the assumptions of the Lemma~\ref{lemma:gradient error}, be $\bm{\theta'}$ and $\bm{\hat{\theta}}$ as defined in Lemma~\ref{lemma: kl bound}, and assuming that the reward is bounded by $r_{\max}$. Then the average return of the $\pi_{\bm{\hat{\theta}}}$ satisfies
\begin{align*}
    J_{\pi}(\bm{\hat{\theta}})
    \geq J_{\pi}(\bm{\theta}) -
    \frac{2 \alpha r_{\max}}{1-\gamma}
\alpha c_3 (\epsilon_f c_1(H) + \epsilon_Q c_2(H))
\end{align*}
\begin{proof}
\vspace{-0.1in}
See Appendix.
\end{proof}
\label{th: policy improvement}
\end{theorem}

Hence, we can provide explicit lower bounds of improvement in terms of model error and function error. Theorem~\ref{th: policy improvement} extends previous work of monotonic improvement for model-free policies~\citep{trpo, Kakade02approximatelyoptimal}, to the model-based and actor critic set up by taking the error on the learned functions into account. From this bound one could, in principle, derive the optimal horizon $H$ that minimizes the gradient error. However, in practice, approximation errors are hard to determine and we treat $H$ as an extra hyper-parameter. In section~\ref{sec:grad error}, we experimentally analyze the error on the gradient for different estimators and values of $H$.

\subsection{Algorithm}
Based on the previous sections, we develop a new algorithm that explicitly optimizes the model-augmented actor-critic (MAAC) objective. The overall algorithm is divided into three main steps: model learning, policy optimization, and Q-function learning. 


\begin{algorithm}[t] 
\caption{MAAC}
\label{alg1} 
\begin{algorithmic}[1] 
    \STATE Initialize the policy $\pi_{\bm{\theta}}$, model $\hat{f}_{\bm{\phi}}$, $\hat{Q}_{\bm{\psi}}$,  $\mathcal{D_\text{env}}\leftarrow \emptyset$, and the model dataset $\mathcal{D_\text{model}}\leftarrow \emptyset$
    \REPEAT
    	 \STATE Sample trajectories from the real environment with policy $\pi_{\theta}$. Add them to $\mathcal{D_\text{env}}$.
    	 \FOR{$i = 1 \dots G_1$}
    	 \STATE $\bm{\phi} \leftarrow \bm{\phi} - \beta_f \nabla_{\bm{\phi}}J_f(\bm{\phi})$ using data from $\mathcal{D_\text{env}}$.
    	 \ENDFOR
         \STATE Sample trajectories $\mathcal{T}$ from  $\hat{f}_{\bm{\phi}}$. Add them to $\mathcal{D_\text{model}}$.
         \STATE $\mathcal{D} \leftarrow \mathcal{D_\text{model}} \cup \mathcal{D_\text{env}} $
         \FOR{$i = 1 \dots G_2$}
         \STATE Update $\bm{\theta} \leftarrow \bm{\theta} + \beta_{\pi}~ \nabla_{\bm{\theta}} J_{\pi}(\bm{\theta})$ using data from $\mathcal{D}$
         \STATE Update $\bm{\psi} \leftarrow \bm{\psi} - \beta_{Q}~ \nabla_{\bm{\psi}} J_{Q}(\bm{\psi})$ using data from $\mathcal{D}$
         \label{algo1:outer_update}
         \ENDFOR

    \UNTIL{the policy performs well in the real environment}
    \RETURN Optimal parameters $\bm{\theta^*}$
\end{algorithmic}
\end{algorithm}

\textbf{Model learning. }In order to prevent overfitting and overcome model-bias~\citep{deisenroth2011pilco}, we use a bootstrap ensemble of dynamics models $\{ \hat{f}_{\bm{\phi}_1}, ..., \hat{f}_{\bm{\phi}_M} \}$. Each of the dynamics models parameterizes the mean and the covariance of a Gaussian distribution with diagonal covariance. The bootstrap ensemble captures the epistemic uncertainty, uncertainty due to the limited capacity or data, while the probabilistic models are able to capture the aleatoric uncertainty~\citep{chua2018deep}, inherent uncertainty of the environment. We denote by $f_{\bm{\phi}}$ the transitions dynamics resulting from $\bm{\phi}_{U}$, where $U \sim \mathcal{U}[M]$ is uniform random variable on $\{1, ..., M \}$. The dynamics models are trained via maximum likelihood with early stopping on a validation set. 

\textbf{Policy Optimization. } We extend the MAAC objective with an entropy bonus~\citep{haarnoja2018sacapp}, and perform policy learning by maximizing
\begin{align*}
        J_{\pi}(\bm{\theta}) = \mathbb{E}\left[ \sum_{t=0}^{H-1} \gamma^t r(\hat{s}_t) + \gamma^H Q_{\bm{\psi}}(\hat{s}_H, a_H)\right] + \beta \mathcal{H}(\pi_{\bm{\theta}})
\end{align*}

where $\hat{s}_{t+1} \sim f_{\bm{\phi}}(\hat{s}_t, a_t)$, $\hat{s}_0 \sim \mathcal{D}$, $a \sim \pi_{\bm{\theta}}$. We learn the policy by using the pathwise derivative of the model through $H$ steps and the Q-function by sampling multiple trajectories from the same $\hat{s}_0$. Hence, we learn a maximum entropy policy using pathwise derivative of the model through $H$ steps and the Q-function. We compute the expectation by sampling multiple actions and states from the policy and learned dynamics, respectively.

\textbf{Q-function Learning. } In practice, we train two Q-functions~\citep{fujimoto2018addressing} since it has been experimentally proven to yield better results. We train both Q functions by minimizing the Bellman error (Section~\ref{sec:back-rl}):
\begin{align*}
    J_Q{(\bm{\psi}}) = \mathbb{E}[(Q_{\bm{\psi}}(s_t, a_t) - (r(s_t, a_t) + \gamma Q_{\bm{\psi}}(s_{t+1}, a_{t+1})))^2]
\end{align*}

Similar to~\citep{janner2019mbpo}, we minimize the Bellman residual on states previously visited and imagined states obtained from unrolling the learned model. Finally, the value targets are obtained in the same fashion the Stochastic Ensemble Value Expansion~\citep{buckman2018steve}, using $H$ as a horizon for the expansion. In doing so, we maximally make use of the model by not only using it for the policy gradient step, but also for training the Q-function.
% Finally, we obtain more accurate estimates on the Q-function by training it on data points sampled from the model~\citep{janner2019mbpo}, thus reducing the distributional shift when computing its gradient on a predicted state $H$ steps ahead~\citep{feinberg2018model}.

Our method, MAAC, iterates between collecting samples from the environment, model training, policy optimization, and Q-function learning. A practical implementation of our method is described in Algorithm~\ref{alg1}. First, we obtain trajectories from the real environment using the latest policy available. Those samples are appended to a replay buffer $\mathcal{D}_{\text{env}}$, on which the dynamics models are trained until convergence. The third step is to collect imaginary data from the models: we collect $k$-step transitions by unrolling the latest policy from a randomly sampled state on the replay buffer. The imaginary data constitutes the $\mathcal{D}_{\text{model}}$, which together with the replay buffer, is used to learn the Q-function and train the policy.

Our algorithm consolidates the insights built through the course of this paper, while at the same time making maximal use of recently developed actor-critic and model-based methods. All in all, it consistently outperforms previous model-based and actor-critic methods. 

==> Model-Based Done Right/sections/05_results.tex <==

\section{Results}

Our experimental evaluation aims to examine the following questions: 1) How does MAAC compares against state-of-the-art model-based and model-free methods? 2) Does the gradient error correlate with the derived bound?, 3) Which are the key components of its performance?, and 4) Does it benefit from planning at test time?

In order to answer the posed questions, we evaluate our approach on model-based continuous control benchmark tasks in the MuJoCo simulator~\citep{2012mujoco, wang2019mbbench}.

\subsection{Comparison Against State-of-the-Art}
We compare our method on sample complexity and asymptotic performance against state-of-the-art model-free (MF) and model-based (MB) baselines. Specifically, we compare against the model-free soft actor-critic (SAC)~\citep{haarnoja2018soft}, which is an off-policy algorithm that has been proven to be sample efficient and performant; as well as two state-of-the-art model-based baselines: model-based policy-optimization (MBPO)~\citep{janner2019mbpo} and stochastic ensemble value expansion (STEVE)~\citep{buckman2018steve}. The original STEVE algorithm builds on top of the model-free algorithm DDPG~\citep{lillicrap2015continuous}, however this algorithm is outperformed by SAC. In order to remove confounding effects of the underlying model-free algorithm, we have implemented the STEVE algorithm on top of SAC. We also add SVG(1)~\citep{heess2015learning} to comparison, which similar to our method uses the derivative of dynamic models to learn the policy.
% In order to compare the effect of policy optimization method of SVG(1) and MAAC, we implemented a modified version of SVG(1): follow its way to do policy optimization and do not use the dynamic models to augment dataset, but remain the Q-learning and model-training part the same as we do in MAAC. 

The results, shown in Fig.~\ref{fig:comparison}, highlight the strength of MAAC in terms of performance and sample complexity. 
MAAC scales to higher dimensional tasks while maintaining its sample efficiency and asymptotic performance. In all the four environments, our method learns faster than previous MB and MF methods. 
We are able to learn near-optimal policies in the half-cheetah environment in just over 50 rollouts, while previous model-based methods need at least the double amount of data. Furthermore, in complex environments, such as ant, MAAC achieves near-optimal performance within 150 rollouts while other take orders of magnitudes more data.

\begin{figure}[H]
    \centering
    \includegraphics[trim={2.5cm .5cm 2.5cm 7.5cm}, clip,
    width=\textwidth]{sections/comparison.png}
    \caption{\small Comparison against state-of-the-art model-free and model-based baselines in four different MuJoCo environments. Our method, MAAC, attains better sample efficiency and asymptotic performance than previous approaches. The gap in performance between MAAC and previous work increases as the environments increase in complexity.}
    \label{fig:comparison}
        \vspace{-0.1in}
\end{figure}

\begin{wrapfigure}{R}{0.5\textwidth}
    \centering
    % \vspace{-0.75in}
    \includegraphics[trim={10cm .5cm 10cm 10cm}, clip, width=\linewidth]{sections/toy.jpg}
    \caption{\small $L1$ error on the policy gradient when using the proposed objective for different values of the horizon $H$ as well as the error obtained when using the true dynamics. The results correlate with the assumption that the error in the learned dynamics is lower than the error in the Q-function, as well as they correlate with the derived bounds.}
    \label{fig:error gradient}
    \vspace{-0.5in}
\end{wrapfigure}

\subsection{Gradient Error} \label{sec:grad error}

Here, we investigate how the bounds obtained relate to the empirical performance. In particular, we study the effect of the horizon of the model predictions on the gradient error. In order to do so, we construct a double integrator environment; since the transitions are linear and the cost is quadratic for a linear policy, we can obtain the analytic gradient of the expect return.

Figure~\ref{fig:error gradient} depicts the $L1$ error of the MAAC objective for different values of the horizon $H$ as well as what would be the error using the true dynamics. As expected, using the true dynamics yields to lower gradient error since the only source comes from the learned Q-function that is weighted down by $\gamma ^H$. The results using learned dynamics correlate with our assumptions and the derived bounds: the error from the learned dynamics is lower than the one in the Q-function, but it scales poorly with the horizon. For short horizons the error decreases as we increase the horizon. However, large horizons is detrimental since it magnifies the error on the models.

\subsection{Ablations}
In order to investigate the importance of each of the components of our overall algorithm, we carry out an ablation test. Specifically, we test three different components: 1) not using the model to train the policy, i.e., set $H=0$, 2) not using the STEVE targets for training the critic, and 3) using a single sample estimate of the path-wise derivative.



The ablation test is shown in Figure~\ref{fig:ablation}. The test underpins the importance of backpropagating through the model: setting $H$ to be 0 inflicts a severe drop in the algorithm performance. On the other hand, using the STEVE targets results in slightly more stable training, but it does not have a significant effect. Finally, while single sample estimates can be used in simple environments, they are not accurate enough in higher dimensional environments such as ant.
\begin{figure}[H]
    % \vspace{-0.2 in}
    \centering
    \includegraphics[trim={7.5cm .5cm 7.5cm 7.5cm}, clip ,width=\textwidth]{sections/ablation.jpg}
    \caption{\small Ablation test of our method. We test the importance of several components of our method: not using the model to train the policy ($H=0$), not using the STEVE targets for training the Q-function (-STEVE), and using a single sample estimate of the pathwise derivative. Using the model is the component that affects the most the performance, highlighting the importance of our derived estimator. }
    \label{fig:ablation}
\end{figure}

\subsection{Model Predictive Control}~\label{sec:mpc}
One of the key benefits of methods that combine model-based reinforcement learning and actor-critic methods is that the optimization procedure results in a stochastic policy, a dynamics model and a Q-function. Hence, we have all the components for, at test time, refine the action selection by the means of model predictive control (MPC). Here, we investigate the improvement in performance of planning at test time. Specifically, we use the cross-entropy method with our stochastic policy as our initial distributions. The results, shown in Table~\ref{table:mpc-comp}, show benefits in online planning in complex domains; however, its improvement gains are more timid in easier domains, showing that the learned policy has already interiorized the optimal behaviour.

\begin{table}[h!]
\begin{center}
 \begin{tabular}{|c|| c| c| c| c|} 
 \hline
  & AntEnv & HalfCheetahEnv & HopperEnv & Walker2dEnv \\ [0.5ex] 
 \hline\hline
MAAC+MPC & $3.97\text{e}3 \pm 1.48\text{e}3$ & $1.09\text{e}4 \pm 94.5$ & $2.8\text{e}3 \pm 11$ & $1.76\text{e}3 \pm 78$ \\ 
 \hline
 MAAC & $3.06\text{e}3 \pm 1.45\text{e}3$ &$1.07\text{e}4 \pm 253$ & $2.77\text{e}3 \pm 3.31$ & $1.61\text{e}3 \pm 404$ \\
 \hline

\end{tabular}
\end{center}
 \caption{Performance at test time with (maac+mpc) and without (maac) planning of the converged policy using the MAAC objective.}
 \label{table:mpc-comp}
\end{table}

==> Model-Based Done Right/sections/06_conclusion.tex <==

\section{Conclusion}

In this work, we present model-augmented actor-critic, MAAC, a reinforcement learning algorithm that makes use of a learned model by using the pathwise derivative across future timesteps. We prevent instabilities arisen from backpropagation through time by the means of a terminal value function. The objective is theoretically analyzed in terms of the model and value error, and we derive a policy improvement expression with respect to those terms. Our algorithm that builds on top of MAAC is able to achieve superior performance and sample efficiency than state-of-the-art model-based and model-free reinforcement learning algorithms. For future work, it would be enticing to deploy the presented algorithm on a real-robotic agent.


